Genericity Through Stratification

A fundamental issue in the $\lambda$-calculus is to find appropriate notions for meaningfulness. It is well-known that in the call-by-name $\lambda$-calculus (CbN) the meaningful terms can be identified with the solvable ones, and that this notion is not appropriate in the call-by-value $\lambda$-calculus (CbV). This paper validates the challenging claim that yet another notion, previously introduced in the literature as potential valuability, appropriately represents meaningfulness in CbV. Akin to CbN, this claim is corroborated by proving two essential properties. The first one is genericity, stating that meaningless subterms have no bearing on evaluating normalizing terms. To prove this (which was an open problem), we use a novel approach based on stratified reduction, indifferently applicable to CbN and CbV, and in a quantitative way. The second property concerns consistency of the smallest congruence relation resulting from equating all meaningless terms. While the consistency result is not new, we provide the first direct operational proof of it. We also show that such a congruence has a unique consistent and maximal extension, which coincides with a well-known notion of observational equivalence. Our results thus supply the formal concepts and tools that validate the informal notion of meaningfulness underlying CbN and CbV.

==> 6_Proofs/gen_TaxSSim_Decompose.tex <==
\begin{proof}
By induction on the length of the proof of
$\genThHaxTail[\genThHaxSSim]{t}{u}$. Cases on the last rule applied:
\begin{itemize}
\item[\bltI] $(\genThHaxConvSymbSSim)$: Then
    $\genThHaxTail[\genThHaxDSim]{t}{u}$ and we set $\genCCtxt :=
    \Hole$, $t' := t$ and $u' := u$ which concludes this case since $t
    = \Hole\CtxtPlug{t} = \genCCtxt<t'>$, $u = \Hole\CtxtPlug{u} =
    \genCCtxt<u'>$ and $\genThHaxTail[\genThHaxDSim]{t'}{u'}$ by
    hypothesis.

\item[\bltI] $(\genThHaxCtxtSymbSSim)$: Then $t = \genCCtxt''<t''>$
    and $u = \genCCtxt''<u''>$ for some terms $t', u' \in
    \setGenTerms$ such that $\genThHaxTail[\genThHaxSSim]{t''}{u''}$.
    By \ih, there exists a context $\genCCtxt'$ and terms $t', u' \in
    \setCbnTerms$ such that $t'' = \genCCtxt'<t'>$, $u'' =
    \genCCtxt'<u'>$ and $\genThHaxTail[\genThHaxDSim]{t'}{u'}$. We set
    $\genCCtxt := \genCCtxt''<\genCCtxt'>$ which concludes this case
    since $t = \genCCtxt''<t''> = \genCCtxt''<\genCCtxt'<t'>> =
    (\genCCtxt''<\genCCtxt'>)\CtxtPlug{t'} = \genCCtxt<t'>$ and $u =
    \genCCtxt''<u''> = \genCCtxt''<\genCCtxt'<u'>> =
    (\genCCtxt''<\genCCtxt'>)\CtxtPlug{t'} = \genCCtxt<u'>$.
    \qedhere
\end{itemize}
\end{proof}

==> 6_Proofs/gen_Tax_Decompose.tex <==
\begin{proof} ~
\begin{enumerate}
\item By induction on the length of the proof of
    $\genThHaxTail{t}{u}$. Cases on the last rule applied:
    \begin{itemize}
    \item[\bltI] $(\genThHaxConvSymbEq)$: Then
        $\genThHaxTail[\genThHaxSSim]{t}{u}$ and we set $n := 0$ with
        $s_0 := t = u$ which concludes this case since using
        $(\genThHaxReflSymbDSim)$ and $(\genThHaxConvSymbSSim)$, one
        has $\genThHaxTail[\genThHaxSSim]{s_0}{s_0}$.

    \item[\bltI] $(\genThHaxTransSymbEq)$: Then $\genThHaxTail{t}{s'}$
        and $\genThHaxTail{s'}{u}$ for some $s' \in \setCbnTerms$. By
        \ih on both, one has $n_1, n_2 \in \mathbb{N}$ and $s_1^0,
        \dots, s_1^{n_1}, s_2^0, \dots, s_2^{n_2} \in \setCbnTerms$
        such that $t = s_1^0$, $s' = s_1^{n_1}$, $s' = s_2^0$, $u =
        s_2^{n_2}$, $\genThHaxTail[\genThHaxSSim]{s_1^i}{s_1^{i+1}}$
        for all $0 \leq i < n_1$ and
        $\genThHaxTail[\genThHaxSSim]{s_2^i}{s_2^{i+1}}$ for all $0
        \leq i < n_2$. We set $n := n_1 + n_2$, $s_i := s_1^i$ for $0
        \leq i \leq n_1$ and $s_{n_1 + i} := s_2^i$ for $0 < i \leq
        n_2$ which concludes this case since $s_1^{n_1} = s' = s_2^0$.
    \end{itemize}

\item By double implication:
    \begin{itemize}
    \item[$(\Rightarrow)$] By induction on the length of the proof of
        $\genThHaxTail[\genThHaxDSim]{t}{u}$. Cases on the last rule
        applied:
        \begin{itemize}
        \item[\bltI] $(\genThHaxReflSymbDSim)$: Then
            $\genThLambdaTail{t}{u}$ using $(\genThLambdaReflSymb)$.

        \item[\bltI] $(\genThHaxBaseSymbDSim)$: Then $(t, u) \in
            \genThHBaseEquations$. We distinguish two cases:
            \begin{itemize}
            \item[\bltII] $(t, u \in \genThLambdaBaseEquations)$: Then
                $\genThLambdaTail{t}{u}$ using
                $(\genThLambdaStepSymb)$.
            \item[\bltII] $t, u$ meaningless.
            \end{itemize}

        \item[\bltI] $(\genThHaxSymSymbDSim)$: Then
            $\genThHaxTail[\genThHaxDSim]{u}{t}$ and by \ih, one has
            that either $\genThLambdaTail{u}{t}$ or
            $\genThLambdaTail{t}{u}$ from an axiom, or $t$ and $u$ are
            meaningless, thus concluding this case.
        \end{itemize}

    \item[$(\Leftarrow)$] We distinguish three cases:
        \begin{itemize}
        \item[\bltI] $\genThLambdaTail{t}{u}$ from an axiom: We
            distinguish two cases:
            \begin{itemize}
            \item[\bltII] $(\genThLambdaReflSymb)$: Then $t = u$ and
                using $(\genThHaxReflSymbDSim)$, one concludes that
                $\genThHaxTail[\genThHaxDSim]{t}{u}$.

            \item[\bltII] $(\genThLambdaStepSymb)$: Then $(t, u) \in
                \genThLambdaBaseEquations$ thus
                $\genThHaxTail[\genThHaxDSim]{t}{u}$ using
                $(\genThHaxBaseSymbDSim)$.
            \end{itemize}

        \item[\bltI] $\genThLambdaTail{u}{t}$ from an axiom: We
            distinguish two cases:
            \begin{itemize}
            \item[\bltII] $(\genThLambdaReflSymb)$: Then $u = t$ and
                using $(\genThHaxReflSymbDSim)$, one concludes that
                $\genThHaxTail[\genThHaxDSim]{t}{u}$.

            \item[\bltII] $(\genThLambdaStepSymb)$: Then $(t, u) \in
            \genThLambdaBaseEquations$ thus
            $\genThHaxTail[\genThHaxDSim]{t}{u}$ using
            $(\genThHaxBaseSymbDSim)$ and $(\genThHaxSymSymbDSim)$.
            \end{itemize}

        \item[\bltI] $t$ and $u$ are meaningless: Then using
            $(\genThHaxBaseSymbDSim)$, one concludes that
            $\genThHaxTail{t}{u}$.
            \qedhere
        \end{itemize}
    \end{itemize}
\end{enumerate}
\end{proof}

==> 7_Proofs.tex <==
\section{Proofs of Section \victorTodo}

\subsection{Proofs of Consistency of $\genThH$}


\begin{definition}
    Let $\genThTax$ be the theory associated to the calculus $\lambda$
    defined by the following axioms and rules:
    \begin{equation*}
        \begin{array}{c}
            \begin{prooftree}
                \inferGenThTaxRefl{t}{t}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \hypo{t \mapstoR u}
                \inferGenThTaxStep{t}{u}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \inferGenThTaxMean{t}{u}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \hypoGenThTaxDSim{t}{u}
                \inferGenThTaxSym{u}{t}
            \end{prooftree}
        \\[0.35cm]
            \begin{prooftree}
                \hypoGenThTaxDSim{t}{u}
                \inferGenThTaxConvSSim{t}{u}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \hypoGenThTaxSSim{t}{u}
                \inferGenThTaxAbs{\abs{x}{t}}{\abs{x}{u}}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \hypoGenThTaxSSim{t}{u}
                \inferGenThTaxAppR{\app[\,]{t}{s}}{\app[\,]{u}{s}}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \hypoGenThTaxSSim{t}{u}
                \inferGenThTaxAppL{\app[\,]{s}{t}}{\app[\,]{s}{u}}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \hypoGenThTaxSSim{t}{u}
                \inferGenThTaxEsR{t\esub{x}{s}}{u\esub{x}{s}}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \hypoGenThTaxSSim{t}{u}
                \inferGenThTaxEsL{s\esub{x}{t}}{s\esub{x}{u}}
            \end{prooftree}
        \\[0.35cm]
            \begin{prooftree}
                \hypoGenThTaxSSim{t}{u}
                \inferGenThTaxConvEq{t}{u}
            \end{prooftree}
        \hspace{0.5cm}
            \begin{prooftree}
                \hypoGenThTaxEq{t}{s}
                \hypoGenThTaxEq{s}{u}
                \inferGenThTaxTrans{t}{u}
            \end{prooftree}
        \end{array}
    \end{equation*}
    Provability of an equation $t \genThTaxEq u$ (\resp $t
    \genThTaxDSim u$ and $t \genThTaxSSim u$) in $\genThTax$ is
    denoted by $\genThTaxTail{t}{u}$ (\resp
    $\genThTaxTail[\genThTaxDSim]{t}{u}$ and
    $\genThTaxTail[\genThTaxSSim]{t}{u}$).
\end{definition}


% \begin{lemma}
%     \label{lem:Theories_Tax_|-_t_=_u_iff_H_|-_t_=_u}%
%     Let $t, u \in \setCbnTerms$. Then $\thTaxTail{t}{u}$ if and only
%     if $\thHTail{t}{u}$.
% \end{lemma}
% \deliaLu
% \input{6_Proofs/Theories_Tax_|-_t_=_u_iff_H_|-_t_=_u.tex}


% \begin{lemma}
%     \label{lem:Theories_Tax_Decompose}%
%     Let $t, u \in \setCbnTerms$, then
%     \begin{enumerate}
%     \item If $\thTaxTail{t}{u}$, then there exist $n \in \mathbb{N}$
%         and $s_0, \dots, s_k \in \setCbnTerms$ such that $t = s_0$, $u
%         = s_k$ and $\thTaxTail[\thTaxSSim]{s_i}{s_{i+1}}$ for $0 \leq
%         i < k$. \label{lem:Theories_TaxEq_Decompose}%

%     \item $\thTaxTail[\thTaxDSim]{t}{u}$ \;if and only if\;
%         $\thLambdaTail{t}{u}$ or $\thLambdaTail{u}{t}$ from an axiom,
%         or $t$ and $u$ are meaningless.
%         \label{lem:Theories_TaxDSim_Decompose}%
%     \end{enumerate}
% \end{lemma}
% \deliaLu
% \input{6_Proofs/Theories_Tax_Decompose.tex}


% \begin{lemma}
%     \label{lem:Theories_TaxSSim_Decompose}%
%     Let $t, u \in \setCbnTerms$ such that
%     $\thTaxTail[\thTaxSSim]{t}{u}$, then there exist a context
%     $\FCtxt$ and terms $t', u' \in \setCbnTerms$ such that $t =
%     \FCtxt<t'>$, $u = \FCtxt<u'>$ and
%     $\thTaxTail[\thTaxDSim]{t'}{u'}$.
% \end{lemma}
% \deliaLu
% \input{6_Proofs/Theories_TaxSSim_Decompose.tex}


% \begin{axiom}
%     \label{ax:Confluence}%
%     Confluence of $\Arr_F$ for Calculus $\abstractCalculus$.
% \end{axiom}


% \begin{lemma}
%     \label{lem:Theories_lambda_|-_t_=_u_==>_t_has_FNF_iff_u_has_FNF}%
%     Let $t, u \in \setCbnTerms$ such that $\thLambdaTail{t}{u}$. Then
%     $t$ has a $\FCtxt$-normal form if and only if $u$ has a
%     $\FCtxt$-normal form.

%     Moreover, they share the same $\FCtxt$-normal form.
% \end{lemma}
% \deliaLu
% \input{6_Proofs/Theories_𝝀_|-_t_=_u_==>_t_has_FNF_iff_u_has_FNF.tex}


% \begin{axiom}
%     \label{ax:Full_Genericity}%
%     Full Genericity for Calculus $\abstractCalculus$.
% \end{axiom}


% \begin{lemma}
%     \label{lem:Theories_Tax_|-_t_=_u_and_u_FNF_==>_lambda_|-_t_=_u}%
%     If $u \in \setCbnTerms$ has a $\FCtxt$-normal form, then for any
%     $t \in \setCbnTerms$, if $\thTaxTail{t}{u}$ then
%     $\thLambdaTail{t}{u}$.
% \end{lemma}
% \deliaLu
% \input{6_Proofs/Theories_Tax_|-_t_=_u_and_u_FNF_==>_𝝀_|-_t_=_u.tex}


% \begin{lemma}
%     \label{lem:Theories_H_|-_t_=_u_and_u_FNF_==>_lambda_|-_t_=_u}%
%     Let $t, u \in \setCbnTerms$ such that $t$ has a $\FCtxt$-normal
%     form and $\thHTail{t}{u}$, then $\thLambdaTail{t}{u}$.
% \end{lemma}
% \deliaLu
% \begin{proof}
%     Let $t, u \in \setCbnTerms$ such that $t$ has a $\FCtxt$-normal
%     form and $\thHTail{t}{u}$. Then using
%     \Cref{lem:Theories_Tax_|-_t_=_u_iff_H_|-_t_=_u}, one has that
%     $\thTaxTail{t}{u}$ thus $\thLambdaTail{t}{u}$ using
%     \Cref{lem:Theories_Tax_|-_t_=_u_and_u_FNF_==>_lambda_|-_t_=_u}.
% \end{proof}


% \begin{axiom}
%     \label{ax:thLambda_Consistent}%
%     The theory $\thLambda$ is consistent (thus a \lambdaTheoryTxt).
% \end{axiom}


% \begin{corollary}
%     \label{lem:Theories_H_Consistent}%
%     The theory $\thH$ is consistent.
% \end{corollary}
% \deliaLu
% \begin{proof}
%     Since $\thLambda$ is consistent (\Cref{ax:thLambda_Consistent}),
%     using
%     \Cref{lem:Theories_H_|-_t_=_u_and_u_FNF_==>_lambda_|-_t_=_u}, one
%     deduces that $\thH$ is consistent.
% \end{proof}




% \begin{corollary}
%     The theory $\thH$ is a \lambdaTheoryTxt.
% \end{corollary}
% \begin{proof}
%     \victor{By construction of $\thH$, one has that $\thLambda
%     \subseteq \thH$ thus $\thLambda + \thH \subseteq \thH$ and
%     therefore $\thLambda + \thH = \thH$. Using
%     \Cref{lem:Theories_H_Consistent}, one concludes that $\thH$ is a
%     \lambdaTheoryTxt.}
% \end{proof}


% \subsection{Consistency and Sensibility of $\thH*$}

% \begin{definition}
%     The theory $\thH*$ associated with a calculus $\abstractCalculus$
%     is defined as follows:
%     \begin{equation*}
%         \thH* := \{t \thHEq u \vsep \forall\; \FCtxt, \; \FCtxt<t> \text{ meaningful } \Leftrightarrow \FCtxt<u> \text{ meaningful}\}
%     \end{equation*}
% \end{definition}


% \begin{axiom}
%     \label{ax:Meaningfulness_Stable_Reduction}%
%     Let $t, u \in \setCbnTerms$ such that $t \Arr_F u$, then $t$ is
%     meaningful if and only if $u$ is meaningful.
% \end{axiom}


% \begin{axiom}
%     \label{ax:Surface_Genericity}%
%     Surface Genericity for the Calculus $\abstractCalculus$.
% \end{axiom}


% \begin{lemma} ~
%     \label{lem:Subseteq_H*}%
%     \begin{enumerate}
%     \item $\thLambda + \thH* \subseteq \thH*$.
%         \label{lem:lambda_+_H*_Subseteq_H*}%
%     \item $\thH \subseteq \thH*$.
%         \label{lem:H_Subseteq_H*}%
%     \end{enumerate}
% \end{lemma}
% \begin{proof} ~
% \begin{enumerate}
% \item By induction on the length of the proof $\thLambda +
%     \thHTail*{t}{u}$. Cases on the last rule applied:
%     \begin{itemize}
%     \item[\bltI] $(\AReflSymb)$: Then $t$ is equal to $u$ thus
%         $\thHTail*{t}{u}$ trivially holds.

%     \item[\bltI] $(\ABetaSymb)$: Then $t \mapstoR[\SymbBeta] u$. Let
%         $\FCtxt$ be any context. Since $\FCtxt<t> \Arr_F \FCtxt<u>$,
%         one has that $\FCtxt<t>$ is meaningful if and only if
%         $\FCtxt<u>$ is meaningful
%         by~\Cref{ax:Meaningfulness_Stable_Reduction} and therefore
%         $\thHTail*{t}{u}$.

%     \item[\bltI] $(\ASubsSymb)$: Then $t \mapstoR[\SymbSubs] u$. Let
%         $\FCtxt$ be any context. Since $\FCtxt<t> \Arr_F \FCtxt<u>$,
%         one has that $\FCtxt<t>$ is meaningful if and only if
%         $\FCtxt<u>$ is meaningful by
%         \Cref{ax:Meaningfulness_Stable_Reduction} and therefore
%         $\thHTail*{t}{u}$.

%     \item[\bltI] $(\RSymSymb)$: Then $\thLambda + \thHTail*{u}{t}$ and
%         by \ih, one has that $\thHTail*{u}{t}$ and one concludes by
%         symmetry of the logical equivalence.

%     \item[\bltI] $(\RTransSymb)$: Then $\thLambda + \thHTail*{t}{s}$
%         and $\thLambda + \thHTail*{s}{u}$ and by \ih on both, one
%         deduces that $\thHTail*{t}{s}$ and $\thHTail*{s}{u}$
%         respectively. Therefore one concludes by transitivity of the
%         logical equivalence.

%     \item[\bltI] $(\RAbsSymb)$: Then $t = \abs{x}{t'}$, $u =
%         \abs{x}{u'}$ and $\thLambda + \thHTail*{t'}{u'}$. By \ih, one
%         has that $\thHTail*{t'}{u'}$ thus in particular, for any
%         context $\FCtxt$, one deduces that $\FCtxt<t> =
%         \FCtxt<\abs{x}{t'}>$ is meaningful if and only if
%         $\FCtxt<\abs{x}{u'}> = u$ is meaningful so that
%         $\thHTail*{t}{u}$.

%     \item[\bltI] $(\RAppRSymb)$: Then $t = \app{t'}{s}$, $u =
%         \app{u'}{s}$ and $\thLambda + \thHTail*{t'}{u'}$. By \ih, one
%         has that $\thHTail*{t'}{u'}$ thus in particular, for any
%         context $\FCtxt$, one deduces that $\FCtxt<t> =
%         \FCtxt<\app{t'}{s}>$ is meaningful if and only if
%         $\FCtxt<\app{u'}{s}> = u$ is meaningful so that
%         $\thHTail*{t}{u}$.

%     \item[\bltI] $(\RAppLSymb)$: Then $t = \app[\,]{s}{t'}$, $u =
%         \app[\,]{s}{u'}$ and $\thLambda + \thHTail*{t'}{u'}$. By \ih,
%         one has that $\thHTail*{t'}{u'}$ thus in particular, for any
%         context $\FCtxt$, one deduces that $\FCtxt<t> =
%         \FCtxt<\app[\,]{s}{t'}>$ is meaningful if and only if
%         $\FCtxt<\app[\,]{s}{u'}> = u$ is meaningful so that
%         $\thHTail*{t}{u}$.

%     \item[\bltI] $(\REsRSymb)$: Then $t = t'\esub{x}{s}$, $u =
%         u'\esub{x}{s}$ and $\thLambda + \thHTail*{t'}{u'}$. By \ih,
%         one has that $\thHTail*{t'}{u'}$ thus in particular, for any
%         context $\FCtxt$, one deduces that $\FCtxt<t> =
%         \FCtxt<t'\esub{x}{s}>$ is meaningful if and only if
%         $\FCtxt<u'\esub{x}{s}> = u$ is meaningful so that
%         $\thHTail*{t}{u}$.

%     \item[\bltI] $(\REsLSymb)$: Then $t = s\esub{x}{t'}$, $u =
%         s\esub{x}{u'}$ and $\thLambda + \thHTail*{t'}{u'}$. By \ih,
%         one has that $\thHTail*{t'}{u'}$ thus in particular, for any
%         context $\FCtxt$, one deduces that $\FCtxt<t> =
%         \FCtxt<s\esub{x}{t'}>$ is meaningful if and only if
%         $\FCtxt<s\esub{x}{u'}> = u$ is meaningful so that
%         $\thHTail*{t}{u}$.
%     \end{itemize}

%   \item By \Cref{lem:lambda_+_H*_Subseteq_H*} one has that $\thLambda
%     \subseteq \thH*$, then it is sufficient to show that $\thH*$
%     equates all meaningless terms. Let $t, u \in \setCbnTerms$ be both
%     meaningless. By Surface Genericity (\Cref{ax:Surface_Genericity}),
%     one has that $\FCtxt<t>$ is meaningful if and only if $\FCtxt<u>$
%     is meaningful, thus $\thHTail*{t}{u}$.
% \end{enumerate}
% \end{proof}


% \begin{axiom}
%     \label{ax:Exists_Meaningless}%
%     There is a meaningless term in the calculus $\abstractCalculus$.
% \end{axiom}


% \begin{lemma}
%     \label{lem:Theory_H*_Consistent}%
%     The theory $\thH*$ is consistent.
% \end{lemma}
% \begin{proof}
%     Let us first show that there exists a meaningful term.

%     By consistency of $\thH$ (\Cref{lem:Theories_H_Consistent}), there
%     exist $t, u \in \setCbnTerms$ such that $\thHTail{t}{u}$ is not
%     provable. Suppose by absurd that both $t$ and $u$ are meaningless,
%     then $\thHTail{t}{u}$ which would lead to a contradiction. One
%     deduces that either $t$ or $u$ is meaningful. Without any loss of
%     generality, let us suppose that $t$ is meaningful.

%     By \Cref{ax:Exists_Meaningless}, there exists a meaningless term
%     $s \in \setCbnTerms$. Let $\FCtxt = \Hole$, then $\FCtxt<t> = t$
%     is meaningful and $\FCtxt<s> = s$ is meaningless thus
%     $\thHTail*{t}{s}$ is not provable and $\thH*$ is therefore
%     consistent.
% \end{proof}

% \victor{
% \begin{corollary}
%     \label{lem:Theories_H*_Sensible_Lambda_Theory}%
%     The theory $\thH*$ is a sensible \lambdaTheoryTxt.
% \end{corollary}
% \begin{proof}
%     By \Cref{lem:Subseteq_H*}.\ref{lem:lambda_+_H*_Subseteq_H*}, one
%     has that $\thLambda + \thH* \subseteq \thH*$ thus $\thLambda +
%     \thH* = \thH*$. Using \Cref{lem:Theory_H*_Consistent}, one has
%     that $\thH*$ is a \lambdaTheoryTxt and using
%     \Cref{lem:Subseteq_H*}.\ref{lem:H_Subseteq_H*}, one concludes that
%     it is sensible.
% \end{proof}
% }

% \section{Call-by-Name Theories}

% \subsection{Consistency and Sensibility of $\cbnThH$ and $\cbnThH*$}

% Let us first show that the
% \Cref{ax:Confluence,ax:Full_Genericity,ax:thLambda_Consistent,ax:Meaningfulness_Stable_Reduction,ax:Surface_Genericity,ax:Exists_Meaningless}
% hold in the \cbnCalculusSymb-calculus.

% \begin{axiom}
%     The reduction $\cbnArr_F$ is confluent.
% \end{axiom}
% \begin{proof}
%     See \victorTodo[Ref].
% \end{proof}


% \begin{axiom}
%     Full genericity
% \end{axiom}
% \begin{proof}
%     Special case of \victorTodo.
% \end{proof}


% \begin{axiom}
%     The theory $\cbnThLambda$ is consistent.
% \end{axiom}
% \begin{proof}
    
% \end{proof}


% \begin{axiom}
%     Let $t, u \in \setCbnTerms$ such that $t \cbnArr_F u$. Then $t$ is
%     consistent if and only if $u$ is consistent.
% \end{axiom}
% \begin{proof}
    
% \end{proof}



% \begin{axiom}
%     Surface Genericity
% \end{axiom}
% \begin{proof}
%     Special case of \victorTodo.
% \end{proof}



% \begin{axiom}
%     There is a meaningless term in the \cbnCalculusSymb-calculus.
% \end{axiom}
% \begin{proof}
%     The term $\Omega$ is $\cbnArr_S$ divergent thus by
%     \victorTodo[REF], one concludes that it is meaningless.
% \end{proof}




==> cbv_NoSn_Characterization.tex <==
\begin{proof}
Let $\indexK \in \setOrdinals$ and $t \in \setCbvTerms$. We strengthen
the property as follows:
\begin{itemize}
\item[\bltI] $t \in \cbvVrS_\indexK$ if and only if $t$ is a
    $\cbvSymbSurface_\indexK$-normal form and $\cbvVarPred{t}$.

\item[\bltI] $t \in \cbvNeS_\indexK$ if and only if $t$ is a
    $\cbvSymbSurface_\indexK$-normal form and $\neg\cbvAbsPred{t}$ and
    $\neg\cbvVarPred{t}$.

\item[\bltI] $t \in \cbvNoS_\indexK$ if and only if $t$ is a
    $\cbvSymbSurface_\indexK$-normal form.
\end{itemize}
By double implication:
\begin{itemize}
\item[$(\Rightarrow)$] By mutual induction on $t \in \cbvVrS_\indexK$,
    $t \in \cbvNeS_\indexK$ and $t \in \cbvNoS_\indexK$:
    \begin{itemize}
    \item[\bltI] $t \in \cbvVrS_\indexK$: We distinguish two cases:
        \begin{itemize}
        \item[\bltII] $t = x$: Then $t$ is a
            $\cbvSymbSurface_\indexK$-normal form and in particular
            $\cbvVarPred{t}$.

        \item[\bltII] $t = t_1\esub{x}{t_2}$ with $t_1 \in
            \cbvVrS_\indexK$ and $t_2 \in \cbvNeS_\indexK$: By \ih on
            $t_1$ and $t_2$, one has that both are
            $\cbvSymbSurface_\indexK$-normal forms and in particular
            $\cbvVarPred{t_1}$, $\neg\cbvAbsPred{t_2}$ and
            $\neg\cbvVarPred{t_2}$. Thus $t = t_1\esub{x}{t_2}$ is a
            $\cbvSymbSurface_\indexK$-normal form and
            $\cbvVarPred{t}$.
        \end{itemize}

    \item[\bltI] $t \in \cbvNeS_\indexK$: We distinguish three cases: 
        \begin{itemize}
        \item[\bltII] $t = \app{t_1}{t_2}$ with $t_1
            \in\cbvVrS_\indexK$ and $t_2 \in \cbvNoS_\indexK$: Then by
            \ih on $t_1$ and $t_2$, one has that both are
            $\cbvSymbSurface_\indexK$-normal forms and
            $\cbvVarPred{t_1}$. Thus, $t = \app{t_1}{t_2}$ is also a
            $\cbvSymbSurface_\indexK$-normal form and in particular
            $\neg\cbvAbsPred{t}$ and $\neg\cbvVarPred{t}$.

        \item[\bltII] $t = \app{t_1}{t_2}$ with $t_1 \in
            \cbvNeS_\indexK$ and $t_2 \in \cbvNoS_\indexK$: Then by
            \ih on $t_1$ and $t_2$, one has that both are
            $\cbvSymbSurface_\indexK$-normal forms and
            $\neg\cbvAbsPred{t_1}$. Thus, $t = \app{t_1}{t_2}$ is also
            a $\cbvSymbSurface_\indexK$-normal form and in particular
            $\neg\cbvAbsPred{t}$ and $\neg\cbvVarPred{t}$.

        \item[\bltII] $t = t_1\esub{x}{t_2}$ with $t_1, t_2 \in
            \cbvNeS_\indexK$: Then by \ih on $t_1$ and $t_2$, one has
            that both are $\cbvSymbSurface_\indexK$-normal forms and
            $\neg\cbvAbsPred{t_1}$, $\neg\cbvVarPred{t_1}$,
            $\neg\cbvVarPred{t_2}$ and $\neg\cbvVarPred{t_2}$. Thus,
            $t = t_1\esub{x}{t_2}$ is also a
            $\cbvSymbSurface_\indexK$-normal form and in particular
            $\neg\cbvAbsPred{t}$ and $\neg\cbvVarPred{t}$.
        \end{itemize}

    \item[\bltI] $t \in \cbvNoS_\indexK$: We distinguish four cases:
        \begin{itemize}
        \item[\bltII] $t = \abs{x}{t'}$: We distinguish three cases:
            \begin{itemize}
            \item[\bltIII] $\indexK = 0$: Then $t = \abs{x}{t'}$ is a
                $\cbvSymbSurface_0$-normal form.

            \item[\bltIII] $\indexK = \indexI + 1$ and $t' \in
                \cbvNoS_\indexI$ for some $\indexI \in \mathbb{N}$: By
                \ih on $t'$, one has that $t'$ is a
                $\cbvSymbSurface_\indexI$-normal form thus $t = \abs{x}{t'}$
                is a $\cbvSymbSurface_\indexK$-normal form.

            \item[\bltIII] $\indexK = \indexOmega$ and $t' \in
                \cbvNoS_\indexOmega$: By \ih on $t'$, one has that
                $t'$ is a $\cbvSymbSurface_\indexOmega$-normal form
                thus $t = \abs{x}{t'}$ is also a
                $\cbvSymbSurface_\indexOmega$-normal form.
            \end{itemize}

        \item[\bltII] $t \in \cbvVrS_\indexK$: Then by \ih on $t$, it
            is a $\cbvSymbSurface_\indexK$-normal form.

        \item[\bltII] $t \in \cbvNeS_\indexK$: Then by \ih on $t$, it
            is a $\cbvSymbSurface_\indexK$-normal form.

        \item[\bltII] $t = t_1\esub{x}{t_2}$ with $t_1 \in
            \cbvNoS_\indexK$ and $t_2 \in \cbvNeS_\indexK$: Then by
            \ih on $t_1$ and $t_2$, one has that both are
            $\cbvSymbSurface_\indexK$-normal forms and,
            $\neg\cbvAbsPred{t_2}$ and $\neg\cbvVarPred{t_2}$. Thus,
            $t = t_1\esub{x}{t_2}$ is also a
            $\cbvSymbSurface_\indexK$-normal form.
        \end{itemize}
    \end{itemize}

\item[$(\Leftarrow)$] By induction on $t$:
    \begin{itemize}
    \item[\bltI] $t = x$: Then $\cbvVarPred{t}$ and $t \in
    \cbvVrS_\indexK$.

    \item[\bltI] $t = \abs{x}{t'}$: Then $\cbvAbsPred{t}$. We
        distinguish three cases:
        \begin{itemize}
        \item[\bltII] $\indexK = 0$: Then $t = \abs{x}{t'} \in
        \cbvNoS_0$.

        \item[\bltII] $\indexK = \indexI + 1$ for some $\indexI \in
            \mathbb{N}$: Then, $t'$ is necessarily a
            $\cbvSymbSurface_\indexI$-normal form. By \ih on $t'$, one
            has that $t' \in \cbvNoS_\indexI$ thus $t = \abs{x}{t'}
            \in \abs{x}{\cbvNoS_i} \subseteq \cbvNoS_\indexK$.

        \item[\bltII] $\indexK = \indexOmega$: By \ih on $t'$, one has
            that $t' \in \cbvNoS_\indexOmega$ thus $t = \abs{x}{t'}
            \in \abs{x}{\cbvNoS_\indexOmega} \subseteq
            \cbvNoS_\indexOmega$.
        \end{itemize}

    \item[\bltI] $t = \app{t_1}{t_2}$: Then $\neg\cbvAbsPred{t}$ and
        $\neg\cbvVarPred{t}$. Moreover, $t_1$ and $t_2$ are
        necessarily $\cbvSymbSurface_\indexK$-normal forms and
        $\neg\cbvAbsPred{t_1}$. By \ih on $t_2$, one has that $t_2 \in
        \cbvNoS_\indexK$. We distinguish two cases:
        \begin{itemize}
        \item[\bltII] $\cbvVarPred{t_1}$: Then, by \ih on $t_1$, one
            has that $t_1 \in \cbvVrS_\indexK$, thus $t =
            \app{t_1}{t_2} \in \app{\cbvVrS_\indexK}{\cbvNoS_\indexK}
            \subseteq \cbvNeS_\indexK$.

        \item[\bltII] $\neg\cbvVarPred{t_1}$: Then, by \ih on $t_1$,
            one has that $t_1 \in \cbvNeS_\indexK$, thus $t =
            \app{t_1}{t_2} \in \app{\cbvNeS_\indexK}{\cbvNoS_\indexK}
            \subseteq \cbvNeS_\indexK$.
        \end{itemize}

    \item[\bltI] $t = t_1\esub{x}{t_2}$: Then both $t_1$ and $t_2$ are
        necessarily $\cbvSymbSurface_\indexK$-normal forms and,
        $\neg\cbvAbsPred{t_2}$ and $\neg\cbvVarPred{t_2}$. By \ih on
        $t_2$, one has that $t_2 \in \cbvNeS_\indexK$. We distinguish
        three cases:
        \begin{itemize}
        \item[\bltII] $\cbvVarPred{t_1}$: Then, by \ih on $t_1$, one
            has that $t_1 \in \cbvVrS_\indexK$ thus $t =
            t_1\esub{x}{t_2} \in
            \cbvVrS_\indexK\esub{x}{\cbvNeS_\indexK} \subseteq
            \cbvVrS_\indexK$.

        \item[\bltII] $\neg\cbvVarPred{t_1}$ and
            $\neg\cbvAbsPred{t_1}$: Then, by \ih on $t_1$, one has
            that $t_1 \in \cbvNeS_\indexK$ thus $t = t_1\esub{x}{t_2}
            \in \cbvNeS_\indexK\esub{x}{\cbvNeS_\indexK} \subseteq
            \cbvNeS_\indexK$.

        \item[\bltII] otherwise: Then, by \ih on $t_1$, one has that
            $t_1 \in \cbvNoS_\indexK$ thus $t = t_1\esub{x}{t_2} \in
            \cbvNoS_\indexK\esub{x}{\cbvNeS_\indexK} \subseteq
            \cbvNoS_\indexK$.
        \end{itemize}
    \end{itemize}
\end{itemize}
\end{proof}

==> cbv_Typed_Genericity.tex <==
\begin{proof}
By induction on $\cbvCCtxt$:
\begin{itemize}
\item[\bltI] $\cbvCCtxt = \Hole$: Then $\cbvCCtxt<t> = t$ thus
    $\cbvCCtxt<t>$ is meaningless which is impossible since it
    contradicts \Cref{lem:cbvBKRV_characterizes_meaningfulness}.

\item[\bltI] $\cbvCCtxt = \abs{x}{\cbvCCtxt'}$: Then $\Pi$ is
    necessarily of the following form, for some finite set $I$:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_i \cbvTrBKRV \Gamma_i, x : \M_i \vdash \cbvCCtxt'<t> : \tau_i}
            \delims{\left(}{\right)_{i \in I}}
            \inferCbvBKRVAbs{\quad +_{i \in I} \Gamma_i \vdash \abs{x}{\cbvCCtxt'<t>} : \mset{\M_i \typeArrow \tau_i}_{i \in  I} \quad}
        \end{prooftree}
    \end{equation*}
    with $\Gamma = +_{i \in I} \Gamma_i$ and $\sigma = \mset{\M_i
    \typeArrow \tau_i}_{i \in I}$. For each $i \in I$, by \ih on
    $\Pi_i$, one has $\Pi'_i \cbvTrBKRV \Gamma_i, x : \M_i \cbvTrBKRV
    \cbvCCtxt'<u> : \tau_i$ and we set $\Pi'$ as the following
    derivation:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi'_i \cbvTrBKRV \Gamma_i, x : \M_i \vdash \cbvCCtxt'<u> : \tau_i}
            \delims{\left(}{\right)_{i \in I}}
            \inferCbvBKRVAbs{\quad +_{i \in I} \Gamma_i \vdash \abs{x}{\cbvCCtxt'<u>} : \mset{\M_i \typeArrow \tau_i}_{i \in  I} \quad}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\cbvCCtxt = \app{\cbvCCtxt'}{s}$: Then $\Pi$ is
    necessarily of the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \cbvTrBKRV \Gamma_1 \vdash \cbvCCtxt'<t> : \mset{\M \typeArrow \sigma}}
            \hypo{\Pi_2 \cbvTrBKRV \Gamma_2 \vdash s : \M}
            \inferCbvBKRVApp{\Gamma_1 + \Gamma_2 \vdash \app{\cbvCCtxt'<t>}{s} : \sigma}
        \end{prooftree}
    \end{equation*}
    with $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\Pi_1$, one has
    $\Pi'_1 \cbvTrBKRV \Gamma_1 \vdash \cbvCCtxt'<u> : \mset{\M
    \typeArrow \sigma}$ and we set $\Pi'$ as the following derivation:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi'_1 \cbvTrBKRV \Gamma_1 \vdash \cbvCCtxt'<u> : \mset{\M \typeArrow \sigma}}
            \hypo{\Pi_2 \cbvTrBKRV \Gamma_2 \vdash s : \M}
            \inferCbvBKRVApp{\Gamma_1 + \Gamma_2 \vdash \app{\cbvCCtxt'<u>}{s} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\cbvCCtxt = \app[\,]{s}{\cbvCCtxt'}$: Then $\Pi$ is
    necessarily of the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \cbvTrBKRV \Gamma_1 \vdash s : \mset{\M \typeArrow \sigma}}
            \hypo{\Pi_2 \cbvTrBKRV \Gamma_2 \vdash \cbvCCtxt'<t> : \M}
            \inferCbvBKRVApp{\Gamma_1 + \Gamma_2 \vdash \app{s}{\cbvCCtxt'<t>} : \sigma}
        \end{prooftree}
    \end{equation*}
    with $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\Pi_2$, one has
    $\Pi'_2 \cbvTrBKRV \Gamma_2 \vdash \cbvCCtxt'<u> : \M$ and we set
    $\Pi'$ as the following derivation:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \cbvTrBKRV \Gamma_1 \vdash s : \mset{\M \typeArrow \sigma}}
            \hypo{\Pi'_2 \cbvTrBKRV \Gamma_2 \vdash \cbvCCtxt'<u> : \M}
            \inferCbvBKRVApp{\Gamma_1 + \Gamma_2 \vdash \app{s}{\cbvCCtxt'<u>} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\cbvCCtxt = \cbvCCtxt'\esub{x}{s}$: Then $\Pi$ is
    necessarily of the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \cbvTrBKRV \Gamma_1, x : \M \vdash \cbvCCtxt'<t> : \sigma}
            \hypo{\Pi_2 \cbvTrBKRV \Gamma_2 \vdash s : \M}
            \inferCbvBKRVEs{\Gamma_1 + \Gamma_2 \vdash \cbvCCtxt'<t>\esub{x}{s} : \sigma}
        \end{prooftree}
    \end{equation*}
    with $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\Pi_1$, one has
    $\Pi'_1 \cbvTrBKRV \Gamma_1, x : \M \vdash \cbvCCtxt'<u> : \sigma$
    and we set $\Pi'$ as the following derivation:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi'_1 \cbvTrBKRV \Gamma_1, x : \M \vdash \cbvCCtxt'<u> : \sigma}
            \hypo{\Pi_2 \cbvTrBKRV \Gamma_2 \vdash s : \M}
            \inferCbvBKRVEs{\Gamma_1 + \Gamma_2 \vdash \cbvCCtxt'<u>\esub{x}{s} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\cbvCCtxt = s\esub{x}{\cbvCCtxt'}$: Then $\Pi$ is
    necessarily of the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \cbvTrBKRV \Gamma_1, x : \M \vdash s : \sigma}
            \hypo{\Pi_2 \cbvTrBKRV \Gamma_2 \vdash \cbvCCtxt'<t> : \M}
            \inferCbvBKRVEs{\Gamma_1 + \Gamma_2 \vdash s\esub{x}{\cbvCCtxt'<t>} : \sigma}
        \end{prooftree}
    \end{equation*}
    with $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\Pi_2$, one has
    $\Pi_1 \cbvTrBKRV \Gamma_1, x : \M \vdash \cbvCCtxt'<u> : \sigma$
    and we set $\Pi'$ as the following derivation:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \cbvTrBKRV \Gamma_1, x : \M \vdash s : \sigma}
            \hypo{\Pi'_2 \cbvTrBKRV \Gamma_2 \vdash \cbvCCtxt'<u> : \M}
            \inferCbvBKRVEs{\Gamma_1 + \Gamma_2 \vdash s\esub{x}{\cbvCCtxt'<u>} : \sigma}
        \end{prooftree}
    \end{equation*}
\end{itemize}
\end{proof}
